Certifiable Reachability Learning Using a New Lipschitz Continuous Value Function

We propose a new reachability learning framework for high-dimensional nonlinear systems, focusing on reach-avoid problems. These problems require computing the reach-avoid set, which ensures that all its elements can safely reach a target set despite disturbances within pre-specified bounds. Our framework has two main parts: offline learning of a newly designed reachavoid value function, and post-learning certification. Compared to prior work, our new value function is Lipschitz continuous and its associated Bellman operator is a contraction mapping, both of which improve the learning performance. To ensure deterministic guarantees of our learned reach-avoid set, we introduce two efficient post-learning certification methods. Both methods can be used online for real-time local certification or offline for comprehensive certification. We validate our framework in a 12-dimensional crazyflie drone racing hardware experiment and a simulated 10-dimensional highway take-over example.

==> Lipschitz_proof.tex <==
Consider two arbitrary initial states $x_0,x_0'\in\mathbb{R}^n$.
Given an arbitrarily small $\epsilon>0$, there exists a control policy $\bar{\controlpolicy}$ such that $V(x_0) \leq \min_\disturbancepolicy \sup_t \reachavoidmeasure(\xi_{x_0}^{\bar\controlpolicy,\disturbancepolicy},t) + \epsilon.$
Let $\bar{\disturbancepolicy}$ be the worst-case disturbance policy conditioned on $\bar\controlpolicy$. There exists $\bar t$ such that $V(x_0) \leq  \reachavoidmeasure(\xi_{x_0}^{\bar\controlpolicy,\bar\disturbancepolicy},\bar{t}) + 2\epsilon$. We have $V(x_0') \geq  \reachavoidmeasure(\xi_{x_0'}^{\bar\controlpolicy,\bar\disturbancepolicy},\bar{t}) $. 
Combining these inequalities, we have
\begin{equation}
\begin{aligned}
    V(x_0)  &- V(x_0' ) - 2\epsilon 
    \leq  \min\{ \gamma^{\bar{t}} (r(x_{\bar t})-r(x'_{\bar t})),\\
    &\ \ \ \ \min_{\tau=0,...,\bar{t}} \gamma^\tau (c(x_{\bar t}) - c(x'_{\bar t})) \}\\
    &\leq\max\{ L_r \gamma^{\bar{t}}L_f^{\bar{t}}, \max_{\tau=0,...,\bar{t}} L_c \gamma^{\tau}L_f^{\tau } \} \|x_0-x_0'\|.
\end{aligned}
\label{eq:pf_lma_cont_eq4}
\end{equation}
The condition $\gamma L_f <1$ implies that the coefficient in the right-hand side in \eqref{eq:pf_lma_cont_eq4} is upper bounded by 1 for all $\bar{t}$. As a result, $   V(x_0)  - V(x_0' ) - 2\epsilon \leq  L \|x_0-x_0'\|
$. Similarly, we can show that $
    V(x_0')  - V(x_0 ) - 2\epsilon \leq L \|x_0-x_0'\|.
$
Combining these two inequalities, we prove Theorem \ref{lemma:continuity}.


==> formulation_old.tex <==
% \jlnote{front page picture?}
\section{Problem Formulation}
We denote the state of a system by $x\in \mathbb{R}^n$. Define $\mathbf{u}:=\{u_0,u_1,\dots\}$ where $u_t\in\mathcal{U}\subseteq \mathbb{R}^m$ is a sequence of control inputs. We assume $\mathcal{U}$ to be compact sets. Let $\xi_{x}^{\mathbf{u}}(t)$ be the state trajectory evaluated at time $t$, which evolves according to the update rule
\begin{equation}
\begin{aligned}
    \xi_x^{\mathbf{u}}(0) & = x,\\
    \xi_x^{\mathbf{u}}(t+1) &= f(\xi_x^{\mathbf{u}}(t), u_t),\ t\in\mathbb{Z}_+,
\end{aligned}
\end{equation}
where $\mathbb{Z}_+$ is the set of all non-negative integers and the system dynamics $f(\cdot,\cdot ):\mathbb{R}^n\times \mathcal{U}\to \mathbb{R}^n$ is assumed to be Lipschitz continuous in the state. 

Many control problems involving safety-critical systems can be interpreted as driving the system's state to a specific region while satisfying certain safety constraints. This intuition can be formalized by introducing the concept of \emph{target set} as the set of desirable states to reach as well as the concept of \emph{constraint set} as the set of all the states complying with the given constraints. The task is to design control inputs such that even under the worst-case disturbance the system state trajectory hits the target set while staying in the constraint set all times. We represent the target set and constraint set by $\mathcal{T}=\{x\in\mathbb{R}^n: r(x)>0\}$ and $\mathcal{C}=\{x\in\mathbb{R}^n: c(x)>0 \}$, respectively, for some Lipschitz continuous and bounded functions $r(\cdot): \mathbb{R}^n \to \mathbb{R}$ and $c(\cdot):\mathbb{R}^n\to \mathbb{R}$.

At each time instance $t\in\mathbb{Z}_+$, the control input $u_t$ aims to move the state towards the target set while staying inside the constraint set, whereas the disturbance $d_t$ attempts to drive the state away from the target set and the constraint set. In this work, we consider a conservative setting, where at each time instance the control input plays before the disturbance. 



The intuition behind this non-anticipative strategy is that, given two sequences of control inputs sharing the same values for the first $T$ entries, the corresponding entries of the two sequences of disturbance must also be the same, meaning the disturbance cannot use any information about the future control inputs when taking its own action. We denote by $\Phi$ the set of all non-anticipative strategies. Building upon the previous discussion on reach-avoid zero-sum games, we are now ready to define the definition the \emph{reach-avoid set}:
\begin{equation*}
    \begin{aligned}
    \mathcal{RA(T,C)} := &\{x\in\mathbb{R}^n:  \exists \{u_t\}_{t=0}^\infty \textrm{ and } T\ge 0,\\ &\textrm{s.t., } \forall t\in[0,T],\xi_{x}^{\mathbf{u}}(T) \in\mathcal{T}\wedge   \xi_{x}^{\mathbf{u}}(t)\in \mathcal{C}\},
    \end{aligned}
\end{equation*}
where 's.t.' is the abbreviation of the phrase 'such that'. As such, we formalize the problem to be studied in this paper below.
\begin{problem}[Infinite-horizon reach-avoid game]\label{Reach_avoid_problem}
 Let $\mathcal{T}:=\{x\in\mathbb{}{R}^n: r(x)>0\}$ and $\mathcal{C}:=\{x\in\mathbb{R}^n:c(x)>0\}$ be the target and the constraint set, respectively. Find the reach-avoid set $\mathcal{RA(T,C)}$ and an optimal sequence of control inputs $\{u_t\}_{t=0}^\infty$ for each state in $\mathcal{RA(T,C)}$ such that the state trajectory will reach the target set without violating the constraints. 
\end{problem}

\begin{equation*}
\begin{aligned}
    \mathcal{S(T,C)}:=& \{ x\in\mathbb{R}^n:  \exists \{u_t\}_{t=0}^\infty \textrm{ and }T\ge 0,\textrm{s.t., }\forall t\ge 0,\\
    & \xi_x^{\mathbf{u}}(t\in \mathcal{C}) \textrm{ and } \forall t\in [T,\infty), \xi_x^{\mathbf{u}}(t)\in\mathcal{T}
    \}
\end{aligned}
\end{equation*}


==> rpg.tex <==
\section{Learning the New Reach-avoid Value Function}\label{sec:learning}
% In this section, we tackle the problem of computing $\valuefunc$. %We first focus on discrete state and action spaces, and then extend it to high-dimensional continuous spaces, where we use neural networks for efficient approximation. 
% \subsubsection{Discrete state and action spaces}
% With the Bellman equation \eqref{eq:bellman_backup}, we can compute the value function $\valuepure$ by value iteration: Let $\valuepurezero(\cdot):\mathbb{R}^n \to \mathbb{R}$ be a bounded function, we keep applying the following Bellman backup operator
%Suppose that 

%With the Bellman equation \eqref{eq:bellman_backup}, we can compute the value function $\valuepure$ by value iteration: Let $\valuepurezero(\cdot):\mathbb{R}^n \to \mathbb{R}$ be a bounded function, we keep applying the following Bellman backup operator 
%\begin{equation}\label{eq:value_iteration}
%\valuepurekplusone := \Bellmanbackup[\valuepurek],\  \forall k\in\mathbb{Z}_+.
%\end{equation}
%The contractive Bellman equation operator $\Bellmanbackup[\cdot]$ guarantees the convergence of value iteration within a bounded function space \cite{sutton2018reinforcement}, 
% The contractive Bellman backup operator \eqref{eq:bellman_backup}, as defined in \eqref{eq:bellman_backup}, ensures the convergence of value iteration to \eqref{eq:inf_horizon_reach_avoid_problem}, i.e., $\lim_{k\to \infty}\valuepurek = \valuepure$. %The convergence of value iteration follows from []. %The proposed value function \eqref{eq:inf_horizon_reach_avoid_problem} yields the reach-avoid set, the optimal sequence of control inputs, and the worst-case sequence of disturbances.

%In this section, we compute $\valuefunc$ for general nonlinear systems. 
%By the contraction mapping property of our Bellman equation, our new value function $\valuefunc$ is the unique solution to the Bellman equation $V(x) = \Bellmanbackup[V(x)]$, for all $\gamma\in(0,1)$. %This motivates us to compute $\valuefunc$ through solving the following functional optimization problem
By Theorem~\ref{thm:Bellman}, we can compute $\valuefunc$ through solving
\begin{equation}\label{eq:value loss}
    \min_V \|V - \Bellmanbackup[V]\|_2^2.
\end{equation}
%However, a direct optimization of the above problem is computationally intractable for general nonlinear systems \cite{al2008discrete}. 
%To make this functional optimization computationally tractable, 
To make this functional space optimization problem tractable, we approximate $\valuefunc$ as a feedforward neural network (NN) $\NNvalue(\cdot):\mathbb{R}^n\to \mathbb{R}$, where $\theta$ represents the neural network's parameter vector. Let $\xdist$ be a sampling distribution of the state $x$ during training. We can reformulate the problem \eqref{eq:value loss} as% an optimization over $\theta$: 
\begin{equation}\label{eq:nn value loss}
    \min_{\theta} \mathbb{E}_{x\sim \xdist} \|\NNvalue(x) - \Bellmanbackup[\NNvalue(x)]\|^2_2.
\end{equation}
% However, there is still a challenge. 
%Furthermore, we observe that $\Bellmanbackup[\NNvalue(x)]$ can be rewritten as
% Recall the definition of $\Bellmanbackup[\NNvalue(x)]$, 
% \begin{equation}\label{eq:expanding Bellman backup}
% \Bellmanbackup[\NNvalue(x)]=\max_u \min_d\min \big\{ c(x),  \max \{ r(x), \gamma  \NNvalue(f(x,u,d)) \} \big\}.
% \end{equation}
% We can simplify the notation of the above max-min problem by 
Define $\NNQ(x,u,d):= \min \big\{ c(x),  \max \{ r(x), \gamma   \NNvalue(f(x,u,d)) \} \big\}$. 
The Bellman equation in $\eqref{eq:bellman_backup}$ can be rewritten as
\begin{equation}
    \Bellmanbackup[\NNvalue(x)] = \max_u\min_d \NNQ(x,u,d)
\end{equation}
%The evaluation of $\Bellmanbackup[\NNvalue(x)]$ requires solving a max-min problem over the control $u$ and the disturbance $d$. To address this, 
% To solve this complex max-min problem, we first simplify the notation by representing the terms within the bracket compactly as a state-action function $\NNQ(x,u,d)$, defined as 
% \begin{equation*}%\label{eq:Q}
%     \NNQ(x,u,d) \coloneqq \min\big\{ c(x), \max \{r(x), \gamma \NNvalue(f(x,u,d))\} \big\},
% \end{equation*}
With $\NNQ$, we solve \eqref{eq:nn value loss} via max-min deep deterministic policy gradient (DDPG) \cite{li2019robust}. Similar to prior works \cite{hsu2023isaacs,nguyen2024gameplay,li2023learning}, we approximate the optimal control policy $u = \controlpolicy^*(x)$ and the worst-case disturbance policy $d = \disturbancepolicy^*(x,\controlpolicy^*(x))$ by neural network policies $u = \NNcontrolpolicy(x)$ and $d = \NNdisturbancepolicy(x)$, respectively, with $\NNcontrolparam$ and $\NNdisturbanceparam$ being their parameters. We learn $\NNcontrolpolicy, \NNdisturbancepolicy$ and $\NNvalue$ by jointly optimizing the following three loss functions: %(\cdot):\mathbb{R}^n\to \controlspace$
% , with $\NNcontrolparam$ being its parameter vector. %We approximate the disturbance policy as another neural network $\NNdisturbancepolicy(\cdot): \mathbb{R}^n \to \disturbancespace$, where $\NNdisturbanceparam$ is its parameter vector. %We associate $\NNcontrolpolicy$, $\NNdisturbancepolicy$ and $\NNvalue$ the following loss functions, 


%However, expanding the Bellman back up $\Bellmanbackup$, we observe that solving the following problem
% \begin{equation*}
% \begin{aligned}
%     \min_{\theta} \mathbb{E}_{x\sim \xdist} \|&\NNvalue(x) - \\
%     &\min \{ c(x), \gamma\max\{ r(x), \gamma \NNvalue(f(x, u,d))\}\} \|^2_2
% \end{aligned}
% \end{equation*}
% requires 
% However, expanding the Bellman backup operator $\Bellmanbackup$ in \eqref{eq:nn value loss} gives us
% \begin{equation}
    
% \end{equation}


% From the Bellman equation, we can derive a state-action function $\Qgamma(x,u,d)$ that measures how a pair of control $u$ and disturbance $d$ affect the future value at a state $x$:
% \begin{equation*}%\label{eq:Q}
%     \Qgamma(x,u,d) \coloneqq \min\big\{ c(x), \max \{r(x), \gamma \cdot\valuepure(f(x,u,d))\} \big\},
% \end{equation*}
% where $\valuefunc = \max_u\min_d \Qgamma(x,u,d)$. 

% Given a state $x\in\mathbb{R}^n$, we can define an optimal control policy $\pi(\cdot): \mathbb{R}^n \to \controlspace$ by considering $\pi:=\arg\max_u \min _d Q(x,u,d)$. Similarly, we can define the worst-case disturbance policy $\disturbancepolicy(\cdot): \mathbb{R}^n\to \disturbancespace$ by $ \disturbancepolicy:=\arg\min_d Q(x,\policy(x),d)$. 



% \subsubsection{Continuous state and action spaces}
%For continuous state and action space, we can approximate reach-avoid value functions through neural networks and optimize the neural network value function approximations such that it satisfies the Bellman equation. To this end, we apply deep reinforcement learning for efficiently optimizing the neural network approximated value function. Let $\theta$ represent the parameters of the neural network approximating the reach-avoid value function. We denote by $\NNvalue$ the neural network approximated value function. Similarly, we denote the neural network control policy and disturbance policy by $\NNcontrolpolicy$ and $\NNdisturbancepolicy$, respectively.

% Let $\xdist$ be the sampling distribution. 
\begin{enumerate}
    \item For $\NNcontrolpolicy$:\hspace{1pt}
    % \begin{equation*}
    $\max_{\NNcontrolparam} \mathbb{E}_{x \sim \xdist}\  \NNQ(x,\NNcontrolpolicy(x),\NNdisturbancepolicy(x))$
% \end{equation*}
    \item For $\NNdisturbancepolicy$:\hspace{1pt}
% \begin{equation*}
$\min_{\NNdisturbanceparam}\hspace{2pt}\mathbb{E}_{x\sim \xdist}\  \NNQ(x,\NNcontrolpolicy(x), \NNdisturbancepolicy(x))$
% \end{equation*} 
\item For $\NNvalue$:\hspace{6.5pt}
% \begin{equation*}
    $\min_\NNvalueparam  \hspace{5pt}\mathbb{E}_{x\sim \xdist} \|\NNvalue(x) - \NNQ(x, \NNcontrolpolicy(x), \NNdisturbancepolicy(x)) \|_2^2$
    %\min\big\{c(x),\max\big\{r(x), \gamma \NNvalue(f(x,\NNcontrolpolicy(x), \NNdisturbancepolicy(x)))\big\}\big\}\big\|
% \end{equation*}
\end{enumerate}
% Max-min DDPG 

%Under certain conditions on the value function's Lipschitz continuity and neural network representation power, DDPG is guaranteed to converge to an optimal solution \cite{xiong2022deterministic}. However, in practice, it is hard to verify the neural network's representation power, and therefore, 
Though DDPG converges under certain conditions \cite{xiong2022deterministic}, in practice, DDPG can diverge or converge to a sub-optimal solution. 
%However, similar to most deep RL methods, max-min DDPG is not guaranteed to converge to an optimal solution where $\NNvalue(x)$ satisfies the Bellman equation \eqref{eq:bellman_backup}.
When $\NNvalue(x)$ is a suboptimal solution, %fails to satisfy the Bellman equation, 
the super zero-level set of $\NNvalue(x)$ cannot be reliably considered as the reach-avoid set. We propose methods for certifying a trustworthy reach-avoid set in the following section. %We consider the super-zero level set of a suboptimal solution $\NNvalue$ as an approximation of the ground truth reach-avoid set. %In the following section, we propose methods for certifying a set of states that are guaranteed to reach the target set safely for all possible disturbances, even when having training errors.


% Since the Bellman operator \eqref{eq:bellman_backup} is a contraction mapping, there exists a unique global minimizer $\NNvalue$ to the above problem. We apply minimax DDPG \cite{li2019robust} to minimize the above three loss functions alternative. 



% \begin{remark}
%     The convergence of deterministic policy gradient requires Lipschitz continuity of Q function \cite{xiong2022deterministic}. Thanks to Theorem~\ref{lemma:continuity}, our value function is guaranteed to be Lipschitz continuous when $\gamma\in[0,1)$ is sufficiently small. We will show in Section \ref{sec:gamma experiment} that Lipschitz continuity of $\valuefunc$ improves learning stability, which distinguishes our method from existing works whose value functions could be discontinuous. 
% \end{remark}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figure/learned_vs_ground_truth_DI_calibration.png}
%     \caption{Comparing the ground truth, learned and calibrated reach-avoid set of a reach-avoid double integrator example. The super zero level set recovers the exact reach-avoid set, instead of a subset, as shown in \cite{hsusafety}. }
%     \label{fig:enter-label}
% \end{figure}




==> vk_and_brs.tex <==
\section{Computing the Viability Kernel and the Backward Reachable Set}\label{sec:pure_constraint_and_pure_target}
In this section, we show that the designed value function \eqref{eq:inf_horizon_reach_avoid_problem} can be adapted to compute the viability kernel \cite{fisac2019bridging} and the backward reachable set \cite{bansal2020deepreach}. We first present the formal definitions of these notions below.

We adopt the same definition of viability kernel as in \cite{fisac2019bridging}, where the \emph{viability kernel} is defined with respect to a closed set $\bar{\mathcal{C}}=\{x\in\mathbb{R}^n: c (x)\ge 0\}$, i.e., the closure of the constraint set $\mathcal{C}$, as
\begin{equation*}
    \Omega(\mathcal{\bar{C}}):=\{x\in\mathbb{R}^n:\forall \phi\in\Phi , \exists \mathbf{u} , \textrm{s.t., }\xi_{x}^{\mathbf{u},\phi (\mathbf{u})}(t)\in \mathcal{\bar{C}},\forall t\ge 0  \},
\end{equation*}
which contains all states $x$ from which a state trajectory $\xi_x^{\mathbf{u},\phi(\mathbf{u})}$ can be drawn such that $\xi_{x}^{\mathbf{u},\phi(\mathbf
{u})}(t)\in\bar{\mathcal{C}}$, $\forall t>0$. This set is of importance when the control task is to make the system satisfy some safety-critical constraints in real-world applications \cite{fisac2019bridging}.

The \emph{backward-reachable set} \cite{bansal2020deepreach} of a target set $\mathcal{T}=\{x\in\mathbb{R}^n: r(x)>0\}$ is defined as
\begin{equation*}
\begin{aligned}
    \mathcal{R(T)} := \{ x\in\mathbb{R}^n: &\forall \phi\in\Phi,\exists \mathbf{u}, \exists t \ge 0,\textrm{s.t., } \xi_{x}^{\mathbf{u},\phi(\mathbf{u})}(t)\in\mathcal{T}\},
\end{aligned}
\end{equation*}
which includes all states that can be driven towards the target set $\mathcal{T}$ in finite time. The backward reachable set is a useful concept in reachability analysis \cite{bansal2020deepreach} because it specifies the set of states that can be controlled to reach a given target set. For instance, if an airplane is in the backward reachable set of another one, then it indicates that the two planes could collide with each other if they are not properly controlled.

In what follows, we show how the value function \eqref{eq:inf_horizon_reach_avoid_problem} can be adapted to compute the viability kernel and backward-reachable set.

\begin{proposition}\label{theorem:pure_safe}
Assume that $r(x)=-1$ for all $ x\in\mathbb{R}^n$. It holds that $V(x)\le 0$ for all $ x\in\mathbb{R}^n$. In addition, $V(x)=0$ if and only if $x\in\Omega(\mathcal{\bar{C}})$.
\end{proposition}%

\begin{remark}
The value function in Proposition \ref{theorem:pure_safe} could serve as a control barrier function \cite{ames2016control}, from which we can derive a policy keeping the system states within a given set of the state space.
\end{remark}

%\begin{remark}
%Proposition~\ref{theorem:pure_safe} shows that the zero-level set of the induced value function is the $\Omega(\bar{\mathcal{C}})$, where $\bar{\mathcal{C}}$ is the closure of the open set $\mathcal{C}$. For an open constraint set $\mathcal{C}=\{x\in \mathbb{R}^n:c(x)>0\}$, a conservative viability kernel with respect to $\mathcal{C}$ can be learned by substituting an $\epsilon$-conservative constraint function defined as $\tilde{c}(x):=c(x)-\epsilon$ into the constraint function in \eqref{eq:inf_horizon_reach_avoid_problem}, for some $\epsilon>0$, where $\epsilon$ controls the conservativeness of the approximation.
%\end{remark}


Similarly, we can compute the backward-reachable set by substituting particular constraint functions into \eqref{eq:inf_horizon_reach_avoid_problem}.


\begin{proposition}\label{theorem:pure_reach}
Assume that $c(x)=1$ for all $x\in\mathbb{R}^n$. It holds that $V(x)\ge 0$ for all $x\in\mathbb{R}^n$. In addition, $V(x) >  0$ if and only if $x\in \mathcal{R(T)}$.
\end{proposition}

Given the above results, our method provides a new theoretical angle to computing the reach-avoid set, viability kernel, and backward reachable set for infinite-horizon games, where a common value function \eqref{eq:inf_horizon_reach_avoid_problem} can be adaptively used to compute multiple important sets for safety-critical analysis.


